The Impact of Element Ordering on LM Agent Performance

There has been a surge of interest in language model agents that can navigate virtual environments such as the web or desktop. To navigate such environments, agents benefit from information on the various elements (e.g., buttons, text, or images) present. It remains unclear which element attributes have the greatest impact on agent performance, especially in environments that only provide a graphical representation (i.e., pixels). Here we find that the ordering in which elements are presented to the language model is surprisingly impactful--randomizing element ordering in a webpage degrades agent performance comparably to removing all visible text from an agent's state representation. While a webpage provides a hierarchical ordering of elements, there is no such ordering when parsing elements directly from pixels. Moreover, as tasks become more challenging and models more sophisticated, our experiments suggest that the impact of ordering increases. Finding an effective ordering is non-trivial. We investigate the impact of various element ordering methods in web and desktop environments. We find that dimensionality reduction provides a viable ordering for pixel-only environments. We train a UI element detection model to derive elements from pixels and apply our findings to an agent benchmark--OmniACT--where we only have access to pixels. Our method completes more than two times as many tasks on average relative to the previous state-of-the-art.

==> 3_obs.tex <==
\section{Challenges in Generating Observation Representation for Virtual Agents}

% Something about POMDP
% A virtual agent can only partially observe the state in a computer environment. 
Both the observation space and the representation perceived by a virtual agent differs across environments. 
In the web, the observation space might be the webpage content with the raw HTML as a specific content representation.
For desktop applications, the observation space might be a specific application or the entire desktop.
While prior work has found that multimodal representations composed of text and vision perform better than unimodal representations\citep{koh2024visualwebarena, xie2024osworld, cheng2024seeclick}, the efficiency of \textit{specific} representations is still unclear.

\subsection{Accessibility Tree}
The accessibility tree provides a simplified and structured text representation of either a webpage or an application.
While traditionally used for assistive technologies such as screen readers, the accessibility tree has become a popular starting point for many virtual agent representations\citep{koh2024visualwebarena, web-arena, xie2024osworld}.

\paragraph{Challenges}
Generating an accessibility tree like representation suitable for agent navigation is challenging for desktop applications.
Web accessibility trees are relatively standardized;
they are derived from the Document Object Model (DOM)---which all webpages build upon---and follow documented specifications\citep{w3c_wai_aria, wicg_aom}.
The same is not true for OS level accessibility trees.
Availability and formats can differ depending on OS platform and application and the tree can contain millions of tokens\citep{xie2024osworld}.
In some applications, an accessibility tree may simply be unavailable.
% These are big statements that would suck if I was wrong on.

\subsection{Screenshots and Set-of-Mark}
Screenshots provide a straightforward visual representation of the environment and have been effective in various multimodal virtual agents settings \citep{koh2024visualwebarena, xie2024osworld, kapoor2024omniact, gur2024realworld, yan2023gpt4v}.


\paragraph{Challenges}
The inability of existing vision language models to effectively understand complex GUIs is a primary source of agent failures in desktop applications \citep{xie2024osworld}.
Set-of-Mark \citep{set-of-mark}---an approach where individual items in an image are labeled to improve LM reasoning---has emerged as a popular choice for improving an agent's understanding of GUI elements, especially in web \citep{cheng2024seeclick, koh2024visualwebarena, he2024webvoyager} and mobile environments\citep{yan2023gpt4v}.
However, this effectiveness has not translated to desktop applications \citep{xie2024osworld}.
Additionally, whereas the original set-of-mark approach used image segmentation to label items in a screenshot, web approaches require parsing the Document Object Model\citep{koh2024visualwebarena, he2024webvoyager} and mobile approaches require human annotations\citep{yan2023gpt4v}.
Both of these are not natively available in desktop applications.
